Predictability of Machine Learning Algorithms and Related Feature Extraction Techniques

This thesis designs a prediction system based on matrix factorization to predict the classification accuracy of a specific model on a particular dataset. In this thesis, we conduct comprehensive empirical research on more than fifty datasets that we collected from the openml website. We study the performance prediction of three fundamental machine learning algorithms, namely, random forest, XGBoost, and MultiLayer Perceptron(MLP). In particular, we obtain the following results: 1. Predictability of fine-tuned models using coarse-tuned variants. 2. Predictability of MLP using feature extraction techniques. 3. Predict model performance using implicit feedback.

==> chapters/preliminaries.tex <==
This template has been used to publish the thesis of Buijs~\cite{MScBuijs2010} and is originally used for the thesis of Nugteren~\cite{MScNugteren2010}. 

One of the best resources for \LaTeX basics, and advanced constructs, is the \LaTeX wikibook\footnote{To be found at~\url{http://en.wikibooks.org/wiki/LaTeX/}}. Of course colleagues and a good internet search using your favorite search engine can do wonders if you're stuck. 
